Adaptive Nonparametric Clustering

This paper presents a new approach to non-parametric cluster analysis called Adaptive Weights Clustering (AWC). The idea is to identify the clustering structure by checking at different points and for different scales on departure from local homogeneity. The proposed procedure describes the clustering structure in terms of weights \( w_{ij} \) each of them measures the degree of local inhomogeneity for two neighbor local clusters using statistical tests of "no gap" between them. % The procedure starts from very local scale, then the parameter of locality grows by some factor at each step. The method is fully adaptive and does not require to specify the number of clusters or their structure. The clustering results are not sensitive to noise and outliers, the procedure is able to recover different clusters with sharp edges or manifold structure. The method is scalable and computationally feasible. An intensive numerical study shows a state-of-the-art performance of the method in various artificial examples and applications to text data. Our theoretical study states optimal sensitivity of AWC to local inhomogeneity.

==> Chapters/Conclusion.tex <==
% !TEX root = ../AWC.tex

\section{Conclusions}

The proposed procedure AWC systematically exploits the idea of extracting the structural information
about the underlying data distribution from the observed data in terms of adaptive weights 
and uses this information for sensitive clustering.
The method is appealing and computationally feasible, 
the numerical results indicate the state-of-the-art performance of the method. 
Theoretical properties show it optimality in separating of neighbor regions.
